RACCOON: A Retrieval-Augmented Generation Approach for Location Coordinate Capture from News Articles

Geocoding involves automatic extraction of location coordinates of incidents reported in news articles, and can be used for epidemic intelligence or disaster management. This paper introduces Retrieval-Augmented Coordinate Capture Of Online News articles (RACCOON), an open-source geocoding approach that extracts geolocations from news articles. RACCOON uses a retrieval-augmented generation (RAG) approach where candidate locations and associated information are retrieved in the form of context from a location database, and a prompt containing the retrieved context, location mentions and news articles is fed to an LLM to generate the location coordinates. Our evaluation on three datasets, two underlying LLMs, three baselines and several ablation tests based on the components of RACCOON demonstrate the utility of RACCOON. To the best of our knowledge, RACCOON is the first RAG-based approach for geocoding using pre-trained LLMs.

==> relwork_bk.tex <==
\section{Related Work}
\citet{zhang2024survey} is a survey that decomposes location extraction into two categories: ranking and classification approaches.

Ranking-based approaches query a reference database (gazetteers) and re-rank the entries based on features.  Ranking-based approaches generally work by querying a geospatial database or gazetteer using a search system. The resultant candidate entries are then re-ranked based on significant features such as population or feature type. The first location in the re-ranked list is regarded as the output location.

One of the earliest toponym resolution systems is Edinburgh Parser \citep{grover2010use}, capable of both toponym recognition and resolution. The geotagger processes input texts and identifies strings that denote place names. Each place name is queried against a gazetteer using text matching to produce a list of candidate entries. These entries are re-ranked using a set of heuristics including population, feature type, contextual information, locality and clustering of places in a single document. Each of these are scaled from 0-1 using a rule-based system and combined to provide each candidate with a final score. As with a rule-based approach for toponym recognition, this approach is inherently limited by its reliance on manually defined rules, which can struggle with geoparsing ambiguities. While this approach works well for common, highly populated places, features such as population and feature type bias the approach away from more uncommon place names.

The limitations of the rule-based approach led to the development of machine-learning based systems. Whilst sharing a common heuristic-based approach with the rule-based models, machine-learning systems provide these as input to a supervised model. The DM\_NLP model \citep{wang2019dm_nlp} extracts location references by treating toponym recognition as an NER task and applying the commonly used BiLSTM-CRF architecture. Extracted location references are then matched against the GeoNames gazetteer to generate candidate references. The candidate re-ranking process is then formulated as a binary classification problem about whether the location mentions refers to the candidate. The model incorporates features such as textual similarity and candidate features such as popularity and address code level. Contextual similarities between mentions and candidates are also considered by collecting Wikipedia data as a proxy for candidate-side context since GeoNames lacks contextual information.

\citet{halterman2023mordecai} builds upon this foundation with the Mordecai 3 model. The major difference between models is that Wikipedia is not required for contextual information, with RoBERTa-based contextual embeddings being used instead. These transformer embeddings originate from the NER step, which uses the transformer-based spaCy NER. While this approach achieved a strong performance on the GeoWebNews corpus \citep{gritta2018pragmatic}, it was suggested that fine-tuning the transformers to incorporate contextual clues about the correct location would further improve performance. This is because while transformer models such as RoBERTa are pre-trained for NLP tasks, their produced embeddings are not optimised for toponym resolution. Additionally, machine-learning approaches can derive geographic bias from its training data, favouring locations that are over represented in the training corpora \citep{gomes2024fine}.

GeoNorm, proposed by \citet{zhang2023improving} stands as the first toponym resolution model to leverage the transformer model. It can be separated into several components. In the candidate generator, an index is created containing each entry in the GeoNames gazetteer. Location mentions are matched to these names by attempting a search under several matching strategies including exact match, fuzzy match, token match, abbreviation match and country code match. These entries are then sorted by population, with the most populous entries being the input to the candidate reranker. This is a transformer model which encodes the candidate entries with the location mention. These encoded vector representations are concatenated with vectors representing the population and address type of the location. The candidate reranker is trained using these features to produce the most likely candidates that match the location mention. GeoNorm also addresses ambiguity using a novel two stage resolution approach. It is assumed that high level features such as countries or states can be inferred without context. Therefore, GeoNorm is first applied to all locations, with mentions resolved to these high level features accepted. In the second stage, these inferences are used as context to resolve the remaining toponym mentions. While GeoNorm set a state-of-the-art performance for the GeoWebNews dataset, limitations included the ability of the retriever to produce the correct candidate entry. It was suggested that using document level context to filter candidates to those in appropriate countries and states could help with this issue.

\subsection{Classification Approach}

A classification approach is used to make geospatial predictions when the Earth's surface has been discretised into tiny areas. The geocoding system is then trained to classify the location into one of these tiles. Unlike with the ranking based approach, classification based approaches do not rely on geospatial information from gazetteers.

\citet{delozier2015gazetteer} identified that machine learning based classifiers are able to use features of the text surrounding a toponym to effectively perform toponym resolution. However, they identify that these approaches are reliant on gazetteers and are therefor unable to handle unknown place names or locations which do not appear in these geospatial datasets. To offset this issue, they create geospatial clusters from Wikipedia articles containing locational information, associating all text from these pages with the latitude and longitude tagged in the article. Toponyms are resolved by overlaying geospatial clusters for words in the toponym's context and selecting the strongest overlapping point in the distribution. While effective, the model, known as TopoCluster was found to struggle with large geographic entities such as countries. This is because the lack of gazetteer reference means that these models can produce different geospatial representations of the same entity.

Many geocoding models utilise lexical similarity to associate geospatial information in language with coordinates. However, solely focusing on these features and ignoring others such as coordinates and population can limit the amount of features we can extract from text. \citet{gritta2018melbourne} aims to address this using a geographic vector representation of location mentions called MapVec. This vector is obtained by plotting geographic probabilities, derived from population figures onto a world map. A geocoding model called CamCoder uses this vector along with a target location, other location mentions in context and other context words to train a Convolutional Neural Network (CNN) which classifies the target location into one of 7823 tiles on the Earth's surface. \citet{kulkarni2020spatial} introduces MLG, which employs a similar classification based approach using a CNN. A key difference occurs in how MLG does not employ MapVec like CamCoder. Since MapVec employs population signals, it is prone to population bias, where predictions are biased towards higher population locations.


==> results_backup.tex <==
\begin{table*}
\begin{tabular}{p{2.4cm}p{1cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.001cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.001cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
\toprule
\multicolumn{1}{c}{}      & \multicolumn{5}{c}{GeoVirus}                                              & \multicolumn{1}{l}{} & \multicolumn{5}{c}{GeoWebNews}                                            & \multicolumn{1}{l}{} & \multicolumn{5}{c}{LGL}                                                   \\ \cmidrule(lr){2-6} \cmidrule(lr){8-12} \cmidrule(l){14-18} 
\multicolumn{1}{c}{Model} & MErr            & A@161          & CAcc           & AUC            & Num  &                      & MErr            & A@161          & CAcc           & AUC            & Num  &                      & MErr            & A@161          & CAcc           & AUC            & Num  \\ \midrule
Gazetteer Base Model      & 919.89          & 0.697          & 0.889          & 0.402          & 1885 &                      & 873.69          & 0.721          & 0.891          & 0.3411         & 1028 &                      & 1168.79         & 0.633          & 0.859          & 0.381          & 3050 \\
LLM Base Model            & 159.34          & 0.792          & \textbf{0.969} & 0.372          & 1668 &                      & \textbf{107.91} & 0.871          & \textbf{0.998} & 0.248          & 892  &                      & \textbf{203.86} & \textbf{0.901} & 0.976          & 0.224          & 2964 \\
RAG Base Model            & 162.79          & 0.839          & 0.957          & 0.293          & 2165 &                      & 342.34          & 0.885          & 0.971          & 0.133          & 1443 &                      & 472.55          & 0.831          & 0.951          & 0.203          & 4459 \\ \midrule
RACCOON           & \textbf{124.19} & \textbf{0.861} & 0.958          & \textbf{0.270} & 2166 &                      & 207.76          & \textbf{0.903} & 0.986          & \textbf{0.119} & 1439 &                      & 284.10          & 0.849          & \textbf{0.979} & \textbf{0.175} & 4439 \\ \midrule
RACCOON ( - One Candidate Entry)          & 149.80          & 0.808          & 0.957          & 0.306          & 2166 &                      & 266.85          & 0.856          & 0.984          & 0.168          & 1442 &                      & 360.38          & 0.796          & 0.977          & 0.239          & 4444 \\
RACCOON (- Country Assisted Retrieval) & 146.09          & 0.857          & 0.955          & 0.278          & 2167 &                      & 269.96          & 0.897          & 0.976          & 0.126          & 1440 &                      & 524.94          & 0.822          & 0.946          & 0.202          & 4445 \\
RACCOON (- GeoNames Feature Types)     & 131.99          & 0.858          & 0.961          & 0.274          & 2166 &                      & 216.17          & 0.902          & \textbf{0.986} & 0.120          & 1441 &                      & 274.00          & 0.857          & \textbf{0.980} & 0.172          & 4440 \\
RACCOON (- Population Heuristic)       & 135.76          & 0.849          & 0.952          & 0.277          & 2166 &                      & 208.73          & 0.897          & \textbf{0.986} & 0.114          & 1441 & \textbf{}            & 262.43          & 0.844          & \textbf{0.980} & \textbf{0.152} & 4445 \\
RACCOON (- State Level Context)        & 135.80          & 0.860          & 0.958          & 0.273          & 2166 &                      & 209.57          & 0.897          & \textbf{0.986} & 0.116          & 1439 &                      & 284.51          & 0.849          & 0.979          & 0.180          & 4437 \\
RACCOON (Gemini)                                & 129.21          & \textbf{0.859} & \textbf{0.987} & \textbf{0.279} & 2129 &                      & 115.89         & 0.917          & 0.986          & 0.113          & 1310 &                      & 250.58          & 0.864          & 0.979          & 0.161          & 3915 \\
RACCOON (Gemini / One Candidate Entry)          & 132.28          & 0.807          & 0.981          & 0.305          & 2055 &                      & 111.31         & 0.901          & \textbf{0.991} & 0.134          & 1251 &                      & 263.26          & 0.828          & 0.976          & 0.230          & 3601 \\
RACCOON (Gemini / - Country Assisted Retrieval) & 131.45          & 0.848          & 0.980          & 0.286          & 2111 &                      & 130.53         & \textbf{0.927} & 0.983          & 0.109          & 1307 &                      & 349.80          & 0.860          & 0.960          & 0.174          & 3887 \\
RACCOON (Gemini / - GeoNames Feature Types)     & 135.30          & 0.837          & 0.978          & 0.291          & 2110 &                      & 96.86          & 0.904          & 0.990          & 0.126          & 1317 &                      & \textbf{225.58} & 0.865          & \textbf{0.980} & 0.160          & 3910 \\
RACCOON (Gemini / - Population Heuristic)       & 148.85          & 0.840          & 0.982          & 0.286          & 2130 &                      & 108.27         & 0.914          & 0.989          & \textbf{0.104} & 1338 & \textbf{}            & 238.42          & \textbf{0.876} & 0.975          & \textbf{0.134} & 4301 \\
RACCOON (Gemini / - State Level Context)        & \textbf{126.09} & 0.843          & 0.981          & 0.283          & 2126 &                      & \textbf{92.37} & 0.920          & \textbf{0.991} & 0.113          & 1332 &                      & 267.66          & 0.843          & 0.974          & 0.174          & 3917 \\ \hline
\end{tabular}
\caption{Toponym Resolution Results for Gemini Ablations}
\label{tab:my-table}
\end{table*}
